Learning Category Trees for ID-Based Recommendation: Exploring the Power of Differentiable Vector Quantization

Category information plays a crucial role in enhancing the quality and personalization of recommender systems. Nevertheless, the availability of item category information is not consistently present, particularly in the context of ID-based recommendations. In this work, we propose a novel approach to automatically learn and generate entity (i.e., user or item) category trees for ID-based recommendation. Specifically, we devise a differentiable vector quantization framework for automatic category tree generation, namely CAGE, which enables the simultaneous learning and refinement of categorical code representations and entity embeddings in an end-to-end manner, starting from the randomly initialized states. With its high adaptability, CAGE can be easily integrated into both sequential and non-sequential recommender systems. We validate the effectiveness of CAGE on various recommendation tasks including list completion, collaborative filtering, and click-through rate prediction, across different recommendation models. We release the code and data for others to reproduce the reported results.

==> algos/integration.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\begin{minted}[mathescape,escapeinside=||]{python}
from torch import nn
from cadre import Cadre

class Recommender(nn.Module):
    def __init__(self, conf):
        super().__init__()

        |\PyComment{first line: initialization}|
        self.cadre = Cadre(...)
        ...

    def forward(self, items, users):
        ue = self.u_embs(users)
        ie = self.i_embs(items)

        |\PyComment{second line: quantization}|
        ue, ul = self.cadre.u(ue)
        ie, il = self.cadre.i(ie)

        loss = self.pred(ue, ie)

        |\PyComment{third line: loss updating}|
        return loss + \
            (ul+il) * self.conf.omega
\end{minted}
\caption{\label{algo:integration} Three lines of PyTorch-style code modification to integrate \model{} into a recommender.}
\end{algorithm}


==> figures/completion.tex <==
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.7\linewidth]{images/Completion.pdf}
%     \caption{\label{fig:completion} 
%     %An illustration of the integration of the list completion model with proposed \model{} method.
%     Illustration of integrating \model{} into a list completion model.}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=.7\linewidth]{images/Classification.pdf}
%     \caption{\label{fig:classification} 
%     %An overview of cascaded classifier module.
%     Structure of the cascaded classifier.
%     }
% \end{figure}


==> figures/dice.tex <==
% \begin{figure*}
%     \centering
%     % \setlength\tabcolsep{2pt}
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{cc}
%     \multirow{2}{*}{
%     \begin{subfigure}{0.6\linewidth}
%         % \resizebox{\linewidth}{!}{
%             \includegraphics[\linewidth]{images/Cadre.pdf}
%         % }
%         \caption{\label{fig:framework}Dice}
%     \end{subfigure}
%     } &
%     \begin{subfigure}{0.35\linewidth}
%         % \resizebox{1.0\linewidth}{!}{
%             \includegraphics[\linewidth]{images/Non-SeqRec.pdf}
%         % }
%         \caption{\label{fig:non-seq}Non-Sequential Recommendation}
%     \end{subfigure}
%      \\
%     & \begin{subfigure}{0.35\linewidth}
%         % \resizebox{1.0\linewidth}{!}{
%             \includegraphics[\linewidth]{images/SeqRec.pdf}
%         % }
%         \caption{\label{fig:seq}Sequential Recommendation}
%     \end{subfigure}
%     \end{tabular}
%     }
%     \caption{\label{fig:dice} (a) Overview of our proposed differentiable and cascaded vector quantization (Dice) framework.}
% \end{figure*}


\begin{figure*}[t]
  \centering
  \begin{subfigure}[b]{0.55\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/Cadre.pdf}
    \caption{\label{fig:framework}}
  \end{subfigure}%
  \hspace{0.05\textwidth} 
  \begin{subfigure}[b]{0.35\textwidth}
    \centering
    \includegraphics[width=\linewidth]{images/Non-SeqRec.pdf}
    \caption{\label{fig:non-seq}}
    \vspace{20pt}
    \includegraphics[width=\linewidth]{images/SeqRec.pdf}
    \caption{\label{fig:seq}}
  \end{subfigure}
  \caption{\label{fig:dice} (a) Overview of our proposed co-evolving vector quantization (\model{}) framework. (b) Integration of \model{} to non-sequential recommenders. (c) Integration of \model{} to sequential recommenders.}
\end{figure*}


==> figures/fuse.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{images/Fuse-Both.pdf}
    \caption{\label{fig:fuse} 
    Integration of \model{} to recommenders. }
\end{figure}

==> figures/general_and_gnn.tex <==
\begin{figure}[t]
\centering
% \setlength\tabcolsep{2pt}
\begin{tabular}{cc}
\begin{subfigure}{0.45\linewidth}
    \includegraphics[width=1\textwidth]{images/GNN.pdf}
    \caption{\label{fig:general}}
\end{subfigure} & 
\begin{subfigure}{0.45\linewidth}
    \includegraphics[width=1\textwidth]{images/General.pdf}
    \caption{\label{fig:gnn}}
\end{subfigure}
\end{tabular}

\caption{\label{fig:general_and_gnn} 
%An illustration of the integration of the (a) graph-based recommender and (b) general recommender with proposed \model{} method.
Illustration of integrating \model{} into  a graph-based recommender (a) and a general recommender (b).
}
\end{figure}


==> figures/quantizer.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.85\linewidth]{images/Quantizer}
    \caption{\label{fig:quantizer} A general design of vector quantizer module.}
\end{figure}

==> figures/visual.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.5\linewidth]{images/visual.pdf}
    \caption{\label{fig:ex-visual}Visualization of the learned categorization.}
\end{figure}

==> plots/alpha/alpha.tex <==
\begin{figure}
    \centering
    \setlength\tabcolsep{2pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cc}
    \multicolumn{2}{c}{
        \resizebox{1.0\linewidth}{!}{
            \input{plots/alpha/legend}
        }
    } \\
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/alpha/zhihu}
        }
        \caption{\label{fig:alpha-zhihu}Zhihu}
    \end{subfigure} &
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/alpha/goodreads}
        }
        \caption{\label{fig:alpha-goodreads}Goodreads}
    \end{subfigure}
    \end{tabular}
    }
    
    \caption{\label{fig:alpha}
    Impact of the weight of residual add $\alpha$ on the \model{}$_\text{FANS}$ model.
    We use the model with $\alpha=0$ as the reference baseline and measure the \textit{relative improvement} of each metric compared to the baseline for various values of $\alpha$, defined as $(m_\alpha - m_\text{0}) / m_\text{0} * 100\%$, where $m$ is one of the metrics \{N@5, N@10, HR@5, HR@10\}.
    Therefore, the relative improvement of $\alpha=0$ is constant at 0\%.
    }
\end{figure}

==> plots/beta/beta.tex <==
\begin{figure}
    \centering
    \setlength\tabcolsep{2pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cc}
     \multicolumn{2}{c}{
        \resizebox{1.0\linewidth}{!}{
            \input{plots/alpha/legend}
        }
    } \\
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/beta/zhihu}
        }
        \caption{\label{fig:beta-zhihu}Zhihu}
    \end{subfigure} &
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/beta/goodreads}
        }
        \caption{\label{fig:beta-goodreads}Goodreads}
    \end{subfigure}
    \end{tabular}
    }
    
    \caption{\label{fig:beta} Impact of the commitment cost $\beta$ on the \model{}$_\text{FANS}$ model. We use the model with $\beta=0$ as the reference baseline.}
\end{figure}

==> plots/dual.tex <==
\begin{figure}
\centering
\resizebox{0.6\linewidth}{!}{
\begin{tikzpicture}
\begin{axis}[
    ybar,
    ymin=60,
    ymax=75,
    xtick=data,
    xticklabels={DCN, DeepFM, FiBiNET, FinalMLP},
    ylabel=N@5,
    bar width=6pt,
%    xlabel=Models,
    enlarge x limits=0.15,
    legend style={
        at={(0.95,0.05)},
        anchor=south east,
        nodes={scale=0.8, transform shape},
        % draw=none,
        % fill=none,
        /tikz/every even column/.append
        style={column sep=5pt},
    },
]
\addplot[teal!80!black, fill=teal!50!white] coordinates {(1,67.81) (2,66.40) (3,70.16) (4,70.00)};
\addplot[olive!80!black, fill=olive!50!white] coordinates {(1,69.06) (2,69.12) (3,71.88) (4,71.94)};
\addplot[purple!80!black, fill=purple!50!white] coordinates {(1,69.25) (2,68.60) (3,71.56) (4,72.73)};
\addplot[orange!80!black, fill=orange!50!white] coordinates {(1,70.47) (2,70.35) (3,73.28) (4,74.40)};
\legend{Backbone, User \model{}, Item \model{}, Dual \model{}}
\end{axis}
\end{tikzpicture}
}
\caption{\label{fig:ablation-dual} Influence of the use of user and item \model{} in non-sequential recommendation.}
\end{figure}


==> plots/omega_code/omega.tex <==
\begin{figure}
    \centering
    \setlength\tabcolsep{2pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cc}
    \multicolumn{2}{c}{
        \resizebox{1.0\linewidth}{!}{
            \input{plots/alpha/legend}
        }
    } \\
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/omega_code/zhihu}
        }
        \caption{\label{fig:omega_code-zhihu}Zhihu}
    \end{subfigure} &
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/omega_code/goodreads}
        }
        \caption{\label{fig:omega_code-goodreads}Goodreads}
    \end{subfigure}
    \end{tabular}
    }
    
    \caption{\label{fig:omega_code}
    Impact of the weight of codebook classification loss $\omega_\text{code}$ on the \model{}$_\text{FANS}$ model. We use the model with $\omega_\text{code}=0$ as the reference baseline.}
\end{figure}

==> plots/visualize.tex <==
\begin{figure}

\begin{tikzpicture}
    \begin{axis}[
        ylabel=Percentage \%,
        xlabel=$\#Entries$,
        % xtick={0,1,2,3,4,5,6},
        % xticklabels={0, 0.2, 0.4, 0.6, 0.8, 1.0},
        line width=0.35mm,
        grid=both,
        grid style=dashed,
        legend style={
            at={(0.9,0.2)},
            anchor=south east
        }
    ]

        \addplot[
            olive,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ] % lifestyle
            coordinates{
                (1, 15.05)
                (2, 28.42)
                (3, 38.08)
                (4, 46.57)
                (5, 53.73)
                (6, 60.38)
                (7, 65.66)
                (8, 69.01)
                (9, 72.15)
                (10, 74.82)
                (11, 77.00)
                (12, 79.07)
                (13, 80.78)
                (14, 82.38)
                (15, 83.78)
                (16, 85.16)
                (17, 86.46)
                (18, 87.73)
                (19, 88.63)
                (20, 89.33)
                (21, 90.04)
                (22, 90.71)
                (23, 91.31)
                (24, 91.91)
                (25, 92.44)
                (26, 92.95)
                (27, 93.38)
                (28, 93.81)
                (29, 94.25)
                (30, 94.68)
                (31, 95.12)
                (32, 95.55)
                (33, 95.99)
                (34, 96.39)
                (35, 96.76)
                (36, 97.06)
                (37, 97.29)
                (38, 97.49)
                (39, 97.69)
                (40, 97.86)
                (41, 97.99)
                (42, 98.13)
                (43, 98.26)
                (44, 98.40)
                (45, 98.53)
                (46, 98.66)
                (47, 98.76)
                (48, 98.86)
                (49, 98.93)
                (50, 99.00)
                (51, 99.06)
                (52, 99.13)
                (53, 99.20)
                (54, 99.26)
                (55, 99.33)
                (56, 99.40)
                (57, 99.47)
                (58, 99.53)
                (59, 99.60)
                (60, 99.63)
                (61, 99.67)
                (62, 99.70)
                (63, 99.73)
                (64, 99.77)
                (65, 99.80)
                (66, 99.83)
                (67, 99.87)
                (68, 99.90)
                (69, 99.93)
                (70, 99.97)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            };
    \end{axis}
\end{tikzpicture}


\caption{\label{fig:visualize} Categorization quality.}
\end{figure}

==> plots/visualize/deepfm.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ylabel=Percentage \%,
        xlabel=$\#Entries$,
        % xtick={0,1,2,3,4,5,6},
        % xticklabels={0, 0.2, 0.4, 0.6, 0.8, 1.0},
        line width=0.35mm,
        grid=both,
        grid style=dashed,
    ]

        \addplot[
            olive,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ] % lifestyle
            coordinates{
                (1, 29.46)
                (2, 46.31)
                (3, 58.81)
                (4, 68.20)
                (5, 74.06)
                (6, 77.97)
                (7, 81.85)
                (8, 84.95)
                (9, 86.96)
                (10, 88.40)
                (11, 89.74)
                (12, 90.94)
                (13, 92.04)
                (14, 93.11)
                (15, 94.15)
                (16, 95.02)
                (17, 95.89)
                (18, 96.66)
                (19, 97.02)
                (20, 97.36)
                (21, 97.63)
                (22, 97.86)
                (23, 98.09)
                (24, 98.26)
                (25, 98.43)
                (26, 98.60)
                (27, 98.76)
                (28, 98.93)
                (29, 99.03)
                (30, 99.13)
                (31, 99.23)
                (32, 99.30)
                (33, 99.36)
                (34, 99.43)
                (35, 99.47)
                (36, 99.50)
                (37, 99.53)
                (38, 99.57)
                (39, 99.60)
                (40, 99.63)
                (41, 99.67)
                (42, 99.70)
                (43, 99.73)
                (44, 99.77)
                (45, 99.80)
                (46, 99.83)
                (47, 99.87)
                (48, 99.90)
                (49, 99.93)
                (50, 99.97)
                (51, 100.00)
                (52, 100.00)
                (53, 100.00)
                (54, 100.00)
                (55, 100.00)
                (56, 100.00)
                (57, 100.00)
                (58, 100.00)
                (59, 100.00)
                (60, 100.00)
                (61, 100.00)
                (62, 100.00)
                (63, 100.00)
                (64, 100.00)
                (65, 100.00)
                (66, 100.00)
                (67, 100.00)
                (68, 100.00)
                (69, 100.00)
                (70, 100.00)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            };
            
        \addplot[
            orange,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ]  % travel
            coordinates{
                (1, 30.43)
                (2, 47.16)
                (3, 59.71)
                (4, 69.70)
                (5, 75.71)
                (6, 79.79)
                (7, 83.11)
                (8, 85.46)
                (9, 87.45)
                (10, 89.08)
                (11, 90.47)
                (12, 91.77)
                (13, 93.00)
                (14, 93.96)
                (15, 94.86)
                (16, 95.69)
                (17, 96.28)
                (18, 96.81)
                (19, 97.31)
                (20, 97.78)
                (21, 98.04)
                (22, 98.27)
                (23, 98.47)
                (24, 98.67)
                (25, 98.87)
                (26, 99.00)
                (27, 99.14)
                (28, 99.24)
                (29, 99.34)
                (30, 99.40)
                (31, 99.47)
                (32, 99.54)
                (33, 99.60)
                (34, 99.63)
                (35, 99.67)
                (36, 99.70)
                (37, 99.73)
                (38, 99.77)
                (39, 99.80)
                (40, 99.83)
                (41, 99.87)
                (42, 99.90)
                (43, 99.93)
                (44, 99.97)
                (45, 100.00)
                (46, 100.00)
                (47, 100.00)
                (48, 100.00)
                (49, 100.00)
                (50, 100.00)
                (51, 100.00)
                (52, 100.00)
                (53, 100.00)
                (54, 100.00)
                (55, 100.00)
                (56, 100.00)
                (57, 100.00)
                (58, 100.00)
                (59, 100.00)
                (60, 100.00)
                (61, 100.00)
                (62, 100.00)
                (63, 100.00)
                (64, 100.00)
                (65, 100.00)
                (66, 100.00)
                (67, 100.00)
                (68, 100.00)
                (69, 100.00)
                (70, 100.00)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            };

        
        \addplot[
            purple,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ] % weather
            coordinates{
                (1, 28.87)
                (2, 45.44)
                (3, 57.90)
                (4, 68.01)
                (5, 74.05)
                (6, 78.62)
                (7, 82.31)
                (8, 85.27)
                (9, 87.62)
                (10, 89.16)
                (11, 90.70)
                (12, 91.93)
                (13, 93.04)
                (14, 94.08)
                (15, 95.04)
                (16, 95.77)
                (17, 96.46)
                (18, 97.08)
                (19, 97.58)
                (20, 97.96)
                (21, 98.23)
                (22, 98.46)
                (23, 98.65)
                (24, 98.81)
                (25, 98.92)
                (26, 99.04)
                (27, 99.15)
                (28, 99.27)
                (29, 99.35)
                (30, 99.42)
                (31, 99.46)
                (32, 99.50)
                (33, 99.54)
                (34, 99.58)
                (35, 99.62)
                (36, 99.65)
                (37, 99.69)
                (38, 99.73)
                (39, 99.77)
                (40, 99.81)
                (41, 99.85)
                (42, 99.88)
                (43, 99.92)
                (44, 99.96)
                (45, 100.00)
                (46, 100.00)
                (47, 100.00)
                (48, 100.00)
                (49, 100.00)
                (50, 100.00)
                (51, 100.00)
                (52, 100.00)
                (53, 100.00)
                (54, 100.00)
                (55, 100.00)
                (56, 100.00)
                (57, 100.00)
                (58, 100.00)
                (59, 100.00)
                (60, 100.00)
                (61, 100.00)
                (62, 100.00)
                (63, 100.00)
                (64, 100.00)
                (65, 100.00)
                (66, 100.00)
                (67, 100.00)
                (68, 100.00)
                (69, 100.00)
                (70, 100.00)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            }; 

        \addplot[
            teal,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ] % foodanddrink
            coordinates{
                (1, 30.32)
                (2, 47.45)
                (3, 60.01)
                (4, 70.51)
                (5, 76.59)
                (6, 80.21)
                (7, 83.00)
                (8, 85.75)
                (9, 87.64)
                (10, 89.02)
                (11, 90.36)
                (12, 91.58)
                (13, 92.76)
                (14, 93.76)
                (15, 94.62)
                (16, 95.45)
                (17, 96.13)
                (18, 96.70)
                (19, 97.18)
                (20, 97.57)
                (21, 97.85)
                (22, 98.14)
                (23, 98.30)
                (24, 98.43)
                (25, 98.53)
                (26, 98.62)
                (27, 98.72)
                (28, 98.82)
                (29, 98.91)
                (30, 99.01)
                (31, 99.07)
                (32, 99.14)
                (33, 99.20)
                (34, 99.26)
                (35, 99.33)
                (36, 99.39)
                (37, 99.46)
                (38, 99.52)
                (39, 99.55)
                (40, 99.58)
                (41, 99.62)
                (42, 99.65)
                (43, 99.68)
                (44, 99.71)
                (45, 99.74)
                (46, 99.78)
                (47, 99.81)
                (48, 99.84)
                (49, 99.87)
                (50, 99.90)
                (51, 99.94)
                (52, 99.97)
                (53, 100.00)
                (54, 100.00)
                (55, 100.00)
                (56, 100.00)
                (57, 100.00)
                (58, 100.00)
                (59, 100.00)
                (60, 100.00)
                (61, 100.00)
                (62, 100.00)
                (63, 100.00)
                (64, 100.00)
                (65, 100.00)
                (66, 100.00)
                (67, 100.00)
                (68, 100.00)
                (69, 100.00)
                (70, 100.00)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            };
    \end{axis}
\end{tikzpicture}


==> plots/visualize/fibinet.tex <==
\begin{tikzpicture}
    \begin{axis}[
        ylabel=Percentage \%,
        xlabel=$\#Entries$,
        % xtick={0,1,2,3,4,5,6},
        % xticklabels={0, 0.2, 0.4, 0.6, 0.8, 1.0},
        line width=0.35mm,
        grid=both,
        grid style=dashed,
        legend style={
            at={(0.9,0.2)},
            anchor=south east
        }
    ]

        \addplot[
            olive,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ] % lifestyle
            coordinates{
                (1, 15.05)
                (2, 28.42)
                (3, 38.08)
                (4, 46.57)
                (5, 53.73)
                (6, 60.38)
                (7, 65.66)
                (8, 69.01)
                (9, 72.15)
                (10, 74.82)
                (11, 77.00)
                (12, 79.07)
                (13, 80.78)
                (14, 82.38)
                (15, 83.78)
                (16, 85.16)
                (17, 86.46)
                (18, 87.73)
                (19, 88.63)
                (20, 89.33)
                (21, 90.04)
                (22, 90.71)
                (23, 91.31)
                (24, 91.91)
                (25, 92.44)
                (26, 92.95)
                (27, 93.38)
                (28, 93.81)
                (29, 94.25)
                (30, 94.68)
                (31, 95.12)
                (32, 95.55)
                (33, 95.99)
                (34, 96.39)
                (35, 96.76)
                (36, 97.06)
                (37, 97.29)
                (38, 97.49)
                (39, 97.69)
                (40, 97.86)
                (41, 97.99)
                (42, 98.13)
                (43, 98.26)
                (44, 98.40)
                (45, 98.53)
                (46, 98.66)
                (47, 98.76)
                (48, 98.86)
                (49, 98.93)
                (50, 99.00)
                (51, 99.06)
                (52, 99.13)
                (53, 99.20)
                (54, 99.26)
                (55, 99.33)
                (56, 99.40)
                (57, 99.47)
                (58, 99.53)
                (59, 99.60)
                (60, 99.63)
                (61, 99.67)
                (62, 99.70)
                (63, 99.73)
                (64, 99.77)
                (65, 99.80)
                (66, 99.83)
                (67, 99.87)
                (68, 99.90)
                (69, 99.93)
                (70, 99.97)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            };
        % \addlegendentry{Lifestyle}
            
        \addplot[
            orange,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ]  % travel
            coordinates{
                (1, 17.09)
                (2, 29.84)
                (3, 40.46)
                (4, 47.89)
                (5, 55.13)
                (6, 62.23)
                (7, 67.41)
                (8, 70.79)
                (9, 73.78)
                (10, 76.10)
                (11, 78.16)
                (12, 80.19)
                (13, 81.88)
                (14, 83.47)
                (15, 84.97)
                (16, 86.39)
                (17, 87.59)
                (18, 88.72)
                (19, 89.61)
                (20, 90.44)
                (21, 91.20)
                (22, 91.87)
                (23, 92.47)
                (24, 93.03)
                (25, 93.56)
                (26, 94.06)
                (27, 94.56)
                (28, 94.99)
                (29, 95.39)
                (30, 95.75)
                (31, 96.08)
                (32, 96.35)
                (33, 96.58)
                (34, 96.78)
                (35, 96.98)
                (36, 97.18)
                (37, 97.34)
                (38, 97.51)
                (39, 97.68)
                (40, 97.84)
                (41, 97.98)
                (42, 98.11)
                (43, 98.24)
                (44, 98.37)
                (45, 98.51)
                (46, 98.64)
                (47, 98.74)
                (48, 98.84)
                (49, 98.94)
                (50, 99.04)
                (51, 99.10)
                (52, 99.17)
                (53, 99.24)
                (54, 99.30)
                (55, 99.37)
                (56, 99.44)
                (57, 99.50)
                (58, 99.57)
                (59, 99.63)
                (60, 99.70)
                (61, 99.77)
                (62, 99.83)
                (63, 99.87)
                (64, 99.90)
                (65, 99.93)
                (66, 99.97)
                (67, 100.00)
                (68, 100.00)
                (69, 100.00)
                (70, 100.00)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            };
        % \addlegendentry{travel}

        
        \addplot[
            purple,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ] % weather
            coordinates{
                (1, 16.57)
                (2, 30.10)
                (3, 40.91)
                (4, 49.13)
                (5, 56.09)
                (6, 62.40)
                (7, 68.05)
                (8, 71.05)
                (9, 73.86)
                (10, 76.36)
                (11, 78.20)
                (12, 79.93)
                (13, 81.55)
                (14, 82.93)
                (15, 84.28)
                (16, 85.58)
                (17, 86.66)
                (18, 87.62)
                (19, 88.58)
                (20, 89.43)
                (21, 90.16)
                (22, 90.85)
                (23, 91.43)
                (24, 91.96)
                (25, 92.50)
                (26, 93.04)
                (27, 93.54)
                (28, 94.04)
                (29, 94.54)
                (30, 95.00)
                (31, 95.46)
                (32, 95.89)
                (33, 96.31)
                (34, 96.69)
                (35, 97.04)
                (36, 97.31)
                (37, 97.58)
                (38, 97.81)
                (39, 98.04)
                (40, 98.27)
                (41, 98.46)
                (42, 98.62)
                (43, 98.73)
                (44, 98.85)
                (45, 98.96)
                (46, 99.08)
                (47, 99.15)
                (48, 99.23)
                (49, 99.31)
                (50, 99.38)
                (51, 99.46)
                (52, 99.54)
                (53, 99.58)
                (54, 99.62)
                (55, 99.65)
                (56, 99.69)
                (57, 99.73)
                (58, 99.77)
                (59, 99.81)
                (60, 99.85)
                (61, 99.88)
                (62, 99.92)
                (63, 99.96)
                (64, 100.00)
                (65, 100.00)
                (66, 100.00)
                (67, 100.00)
                (68, 100.00)
                (69, 100.00)
                (70, 100.00)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            }; 
        % \addlegendentry{weather}

        \addplot[
            teal,
            line width=1mm,
            opacity=0.7
            % mark=x,
        ] % foodanddrink
            coordinates{
                (1, 17.23)
                (2, 31.35)
                (3, 41.53)
                (4, 49.50)
                (5, 57.09)
                (6, 64.23)
                (7, 69.26)
                (8, 72.53)
                (9, 75.28)
                (10, 77.94)
                (11, 79.99)
                (12, 81.81)
                (13, 83.35)
                (14, 84.82)
                (15, 86.30)
                (16, 87.51)
                (17, 88.70)
                (18, 89.85)
                (19, 90.97)
                (20, 91.74)
                (21, 92.38)
                (22, 92.92)
                (23, 93.44)
                (24, 93.92)
                (25, 94.40)
                (26, 94.84)
                (27, 95.23)
                (28, 95.61)
                (29, 95.97)
                (30, 96.25)
                (31, 96.51)
                (32, 96.77)
                (33, 96.99)
                (34, 97.21)
                (35, 97.37)
                (36, 97.50)
                (37, 97.63)
                (38, 97.76)
                (39, 97.89)
                (40, 98.01)
                (41, 98.14)
                (42, 98.27)
                (43, 98.37)
                (44, 98.46)
                (45, 98.56)
                (46, 98.66)
                (47, 98.75)
                (48, 98.85)
                (49, 98.94)
                (50, 99.04)
                (51, 99.14)
                (52, 99.20)
                (53, 99.26)
                (54, 99.33)
                (55, 99.39)
                (56, 99.46)
                (57, 99.52)
                (58, 99.58)
                (59, 99.62)
                (60, 99.65)
                (61, 99.68)
                (62, 99.71)
                (63, 99.74)
                (64, 99.78)
                (65, 99.81)
                (66, 99.84)
                (67, 99.87)
                (68, 99.90)
                (69, 99.94)
                (70, 99.97)
                (71, 100.00)
                (72, 100.00)
                (73, 100.00)
                (74, 100.00)
                (75, 100.00)
                (76, 100.00)
                (77, 100.00)
                (78, 100.00)
                (79, 100.00)
                (80, 100.00)
                (81, 100.00)
                (82, 100.00)
                (83, 100.00)
                (84, 100.00)
                (85, 100.00)
                (86, 100.00)
                (87, 100.00)
                (88, 100.00)
                (89, 100.00)
                (90, 100.00)
                (91, 100.00)
                (92, 100.00)
                (93, 100.00)
                (94, 100.00)
                (95, 100.00)
                (96, 100.00)
                (97, 100.00)
                (98, 100.00)
                (99, 100.00)
                (100, 100.00)
            };
        % \addlegendentry{foodanddrink}
    \end{axis}
\end{tikzpicture}


==> plots/visualize/legend.tex <==
\begin{tikzpicture}
    \begin{customlegend}[
        legend columns=2,
        legend style={
            align=left,
            draw=none,
            column sep=2ex
        },
        legend entries={
            \textsc{lifestyle},
            \textsc{travel},
            \textsc{weather},
            \textsc{foodanddrink},
        }]
        \addlegendimage{olive,solid,line legend,line width=.5mm,opacity=0.7}
        \addlegendimage{orange,solid,line legend,line width=.5mm,opacity=0.7}
        \addlegendimage{purple,solid,line legend,line width=.5mm,opacity=0.7}
        \addlegendimage{teal,solid,line legend,line width=.5mm,opacity=0.7}
        \end{customlegend}
\end{tikzpicture}

==> plots/visualize/visualize.tex <==
\begin{figure}
    \centering
    % \setlength\tabcolsep{2pt}
    \resizebox{.8\linewidth}{!}{
    \begin{tabular}{cc}
     \multicolumn{2}{c}{
        \resizebox{1.0\linewidth}{!}{
            \input{plots/visualize/legend}
        }
    } \\
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/visualize/fibinet}
        }
        \caption{\label{fig:vis-fibinet}\model{}$_\text{FiBiNET}$}
    \end{subfigure} &
    \begin{subfigure}{0.25\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \input{plots/visualize/deepfm}
        }
        \caption{\label{fig:vis-deepfm}\model{}$_\text{DeepFM}$}
    \end{subfigure}
    \end{tabular}
    }
    
    \caption{\label{fig:visualize} Categorization quality.}
\end{figure}

==> tables/baselines.tex <==
\begin{table}[]
\centering
\renewcommand\arraystretch{1.2}
 
\caption{Baselines}
\label{tab:baselines}

\setlength\tabcolsep{3pt}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|ccc}
\toprule
\textbf{Model} & \textbf{Scenario} & \textbf{Type} & \textbf{Encoder} \\
\midrule
\textbf{Caser} & List Competion & Sequential & CNN~\cite{cnn} \\
\textbf{GRU4Rec} & List Competion & Sequential & GRU~\cite{gru} \\
\textbf{SASRec} & List Competion & Sequential & Transformer~\cite{vaswani2017attention} \\
\textbf{CAR} & List Competion & Sequential & Transformer~\cite{vaswani2017attention} \\
\textbf{BERT4Rec} & List Competion & Sequential & Transformer~\cite{vaswani2017attention} \\
\textbf{FANS} & List Competion & Sequential & Transformer~\cite{vaswani2017attention} \\
\midrule
\textbf{LightGCN} & Collaborative Filtering & Graph-based & GCN~\cite{gcn} \\
\textbf{CFKG} & Collaborative Filtering & Graph-based & \\
\textbf{NeuMF} & Collaborative Filtering & General & MLP \& MF \\
\textbf{BPRMF} & Collaborative Filtering & General & MF \\
\midrule
\textbf{DeepFM} & CTR Prediction & General & MLP \& FM \\
\textbf{DCN} & CTR Prediction & General & MLP \& Cross Net \\
\textbf{PNN} & CTR Prediction & General & MLP \\
\bottomrule
\end{tabular}
}
\end{table}

